A multiphase cubic MARS method for fourth- and higher-order interface tracking of two or more materials with arbitrary topology and geometry

For interface tracking of an arbitrary number of materials in two dimensions, we propose a multiphase cubic MARS method that (a) represents the topology and geometry of the interface via graphs, cycles, and cubic splines, (b) applies to any number of materials with arbitrarily complex topology and geometry, (c) maintains an $(r,h)$-regularity of the interface so that the distance between any pair of adjacent markers is within a user-specified range, (d) distributes the markers adaptively along the interface so that arcs with high curvature are resolved by densely populated markers, and (e) achieves fourth-, sixth-, and eighth-order accuracy both in time and in space.} In particular, all possible types of junctions, which pose challenges to VOF methods and level-set methods, are handled with ease. Results of a variety of benchmark tests confirm the analysis and demonstrate the superior accuracy, efficiency, and versatility of the proposed method.

==> sec/analysis.tex <==
% \subsection{The Yin space as a metric space}
% \label{sec:mars-framework}

The volume of a Yin set $\mathcal{Y}$ is given by
\begin{equation}
  \label{eq:int}
\Vert \mathcal{Y} \Vert := \left|\int_{\mathcal{Y}}d \mathbf{x}\right|,
\end{equation}
where the integral can be interpreted as a Riemann integral
since $\mathcal{Y}$ is semianalytic.
The regularized symmetric difference
 $\oplus:\mathbb{Y}\times\mathbb{Y}\rightarrow\mathbb{Y}$
 is defined as %$\mathcal{P}$ and $\mathcal{Q}$ as
\begin{equation}
  \label{eq:oplus}
  \mathcal{P} \oplus \mathcal{Q} := \left( \mathcal{P}\,\backslash\,
    \mathcal{Q} \right) \,
  \mathop{\cup}\nolimits^{\perp\perp} \,
  \left( \mathcal{Q} \,\backslash \,\mathcal{P} \right),
\end{equation}
which satisfies
\begin{align}
  \label{eq:oplusconst}
  \forall \mathcal{Y} \in \mathbb{Y},&\quad \mathcal{Y}\oplus \mathcal{Y} =
  \emptyset, \quad\emptyset \oplus \mathcal{Y} = \mathcal{Y}; 
  \\
  \label{eq:triinequ}
  \forall \mathcal{P}, \mathcal{Q} \in \mathbb{Y},&\quad \Vert \mathcal{P}
  \oplus \mathcal{Q} \Vert \le \Vert \mathcal{P}\Vert + \Vert \mathcal{Q}\Vert.
\end{align}

It follows from \eqref{eq:int}, \eqref{eq:oplus}, \eqref{eq:oplusconst} and
\eqref{eq:triinequ} that $(\mathbb{Y}, d)$ forms a metric space
where the metric $d \,: \, \mathbb{Y} \times \mathbb{Y}
\rightarrow [0, +\infty)$ is 
\begin{equation}
  \label{eq:metric}
  \forall \mathcal{P}, \mathcal{Q} \in \mathbb{Y},\quad
  d(\mathcal{P}, \, \mathcal{Q})\, := \, \Vert \mathcal{P} \oplus
  \mathcal{Q} \Vert.
\end{equation}

% TOADD: approximating the boundary of a Yin set
% by not-a-knot splines.

\subsection{IT errors of a MARS method}
\label{sec:it-errors-mars}

In light of \eqref{eq:metric},
 the IT error of a MARS method at time $t_n$ is defined as
 \begin{equation}
   \label{eq:totalerror}
   E_{\mathrm{IT}}(t_n) := \Vert \mathcal{M}(t_n) \oplus \mathcal{M}^n \Vert.
 \end{equation}

 \begin{defn}
   \label{def:individualerror}
   Individual IT errors of a $\mathrm{MARS}$ method include the following.
   \begin{itemize}
   \item \emph{The representation error} $E^{\mathrm{REP}}$ 
     is the error caused by
     approximating the initial Yin set $\mathcal{M}(t_0)$ with a discrete
     representation $\mathcal{M}^0$.
   \item \emph{The augmentation error} $E^{\mathrm{AUG}}(t_n)$ 
     is the accumulated
     error of augmenting the Yin sets by $\psi_j$.
   \item \emph{The mapping error} $E^{\mathrm{MAP}}(t_n)$ 
     is the accumulated error
     of approximating the exact flow map $\phi$ with the discrete flow map
     $\varphi_{t_j}^k$.
   \item \emph{The adjustment error} $E^{\mathrm{ADJ}}(t_n)$ 
     is the accumulated
     error of adjusting the mapped Yin sets by $\chi_{j+1}$.
   \end{itemize}
   More precisely, these individual errors at $t_n = t_0 + nk$ are defined as:
   \begin{subequations}
     \label{eq:individualerror}
\begin{align}
E^{\mathrm{REP}}(t_{n})=& \left\Vert \phi_{t_0}^{nk}\left[ \mathcal{M}(t_0), \mathcal{M}^{0} \right] \right\Vert;\\
E^{\mathrm{AUG}}(t_{n})=& \left\Vert \bigoplus\limits^{n-1}_{j=0}\phi_{t_j}^{(n-j)k}\left[ \mathcal{M}_{\psi}^j, \mathcal{M}^j \right] \right\Vert;\\
E^{\mathrm{MAP}}(t_{n})=& \left\Vert \bigoplus\limits^{n}_{j=1} \phi_{t_j}^{(n-j)k}\left[ \phi^k_{t_{j-1}} \mathcal{M}^{j-1}_{\psi}, \varphi_{t_{j-1}}^k \mathcal{M}^{j-1}_{\psi} \right] \right\Vert;\\
E^{\mathrm{ADJ}}(t_{n})=&\left\Vert \bigoplus\limits^{n}_{j=1}\phi_{t_j}^{(n-j)k}\left[ \varphi_{t_{j-1}}^k \mathcal{M}_{\psi}^{j-1}, \mathcal{M}^j \right] \right \Vert,
\end{align}
\end{subequations}
where $\mathcal{M}_{\psi}^j := \psi_j \mathcal{M}^j$ and
$\phi_{t_j}^{(n-j)k}\left[ \cdot,\cdot\right]$ is a shorthand notation
given by
\begin{equation}
  \label{eq:phipq}
  \forall \mathcal{P},\, \mathcal{Q} \in \mathbb{Y},\quad
  \phi_{t_0}^{\tau}\left[ \mathcal{P},\, \mathcal{Q} \right]\, := \,
  \phi_{t_0}^{\tau}\left( \mathcal{P} \right) \oplus
  \phi_{t_0}^{\tau}\left( \mathcal{Q} \right).
\end{equation}
\end{defn}

The IT error of a MARS method is bounded
by the sum of the individual errors in (\ref{eq:individualerror}); 
see \cite[Theorem 3.3]{hu2025:_arms} for a proof of

 \begin{thm}
  \label{thm:errorsplit}
  For a single phase, 
  the IT errors of a MARS method satisfy %\eqref{eq:totalerror} and \eqref{eq:individualerror} 
%  problem defined in Definition \ref{def:interfaceTracking} 
\begin{equation}
  E_{\mathrm{IT}}(t_n) \le E^{\mathrm{REP}}(t_n) + E^{\mathrm{AUG}}(t_n) +
  E^{\mathrm{MAP}}(t_n) + E^{\mathrm{ADJ}}(t_n).
\end{equation}
\end{thm}
% \begin{proof}
%   See \cite[Theorem 3.3]{hu2025:_arms}. 
% \end{proof}


\subsection{The representation error  $E^{\mathrm{REP}}$}
\label{sec:representationError}

By Sec.~\ref{sec:topologyOfCommonBoundary},
 all topological structures
 of the initial condition $\partial{\cal M}(t_0)$
 have been captured in the interface graph. 
By Theorems~\ref{thm:periodicSplineErrorEstimates} and 
 \ref{thm:notaKnotSplineErrorEstimates} 
 in Sec.~\ref{sec:geometryOfCommonBoundary},
 the geometry of $\chi(\Gamma)=\partial{\cal M}(t_0)$
 has been approximated by $\partial {\cal M}^0$
 to fourth-order accurate
 by periodic and not-a-knot cubic splines.
More precisely, $\partial {\cal M}^0$ is homeomorphic to $\partial{\cal M}(t_0)$
 and the distance between 
 corresponding points on $\partial {\cal M}^0$ and 
 $\partial {\cal M}(t_0)$ is $O(h_L^4)$. 
Therefore, we have
\begin{equation}
\label{eq:EREPbound}
E^{\mathrm{REP}}(t_n) =
\biggl\Vert
\phi_{t_0}^{nk}
\bigl[{\cal M}(t_0), {\cal M}^0\bigr]
\biggr\Vert
= O(h_L^4),
\end{equation}
where the first equality follows from (\ref{eq:individualerror}a) 
and the second from 

\begin{lem}
\label{lem:normOfPhiPQ}
Suppose 
$\Upsilon:\partial{\cal P}\to\partial{\cal Q}$
is a homeomorphism
between two Yin sets ${\cal P},{\cal Q}$ 
such that
$\max_{{\mathbf{X}}\in\partial{\cal P}}
\left\|{\mathbf{X}}-
  \Upsilon({\mathbf{X}})\right\|_2=\epsilon$.
Then 
$\left\| \phi_{t_0}^\tau[{\cal P},{\cal Q}]\right\|
= O(\epsilon)$.
\end{lem}
\begin{proof}\revise{
  See that of \cite[Lemma 5.4]{hu2025:_arms}.  \qed}
\end{proof}


\subsection{The augmentation error  $E^{\mathrm{AUG}}$}
\label{sec:augerror}

By Definitions \ref{def:MARS} and \ref{def:ARMS},
 the augmentation operation $\psi_n: \mathbb{Y}\rightarrow \mathbb{Y}$
 consists of adding markers on $\partial\mathcal{M}^j$
 in \ref{en:arms-add} and \ref{en:arms-construct}
 and fitting a new set of cubic splines as the boundary of the Yin set.
%  to enforce the upper bound $h_L$ of chordal length
% or in (ARMS-4) to ensure good conditioning of the not-a-knot splines. 
Being ${\cal C}^3$ at each added marker,
 the new set of cubic splines is exactly the same
 as the original one before adding the new markers; 
 see Fig.~\ref{fig:addingpointonSpline}.
% the spline $\partial\mathcal{M}^j$ satisfies all constraints of 
% $\partial\mathcal{M}_{\psi}^j$, which implies that
% the two splines $\partial\mathcal{M}_{\psi}^j$
% and $\partial\mathcal{M}^j$ are exactly the same. 
Hence (\ref{eq:oplusconst}) yields
 $\Vert \mathcal{M}_{\psi}^j \oplus \mathcal{M}^j \Vert = 0$,
 which, combined with (\ref{eq:individualerror}b), implies
\begin{equation}
  \label{eq:EAUGbound}
  E^{\mathrm{AUG}}(t_n) = 
  \left\Vert \bigoplus\nolimits_{j=0}^{n-1} \phi_{t_j}^{(n-j)k}
  \left[ \mathcal{M}_{\psi}^j, \mathcal{M}^j \right] \right\Vert = 0.
\end{equation}

\begin{figure}
  \centering
  \includestandalone[width=0.5\textwidth]{{\TIKZDIR}addingpointonSpline}
  \caption{Fitting a cubic spline on a marker sequence is equivalent to 
   adding markers from the original spline to the marker sequence, 
   reconstructing the spline, and requiring $\mathcal{C}^3$ continuity 
   at those added markers.
  }
  \label{fig:addingpointonSpline}
\end{figure}


\subsection{The mapping error  $E^{\mathrm{MAP}}$}
\label{sec:mappingerror}

The analysis of $E^{\mathrm{MAP}}$
 entails the comparison of the fully discrete flow map $\varphi$
 with the exact flow map $\phi$.
By (\ref{eq:individualerror}c),
it is essential to estimate the mapping error 
within a single time step.
The key challenge lies in estimating
% the maximum distance
% between corresponding points
% on $\partial\phi^k_{t_{j-1}}\mathcal{M}_\psi^{j-1}$
% and the spline $\partial\varphi^k_{t_{j-1}}\mathcal{M}_\psi^{j-1}$,
% which is formally defined as
\begin{equation}
  \label{eq:keyMappingError}
  \begin{array}{l}
    \epsilon_j^{\mathrm{MAP}}
    :=\max_{\mathbf{X}\in\partial\mathcal{M}_\psi^{j-1}}
    \left\|\phi^k_{t_{j-1}}\mathbf{X}
    -\varphi^k_{t_{j-1}}\mathbf{X}\right\|_2
  \end{array}
\end{equation}
since Lemma \ref{lem:normOfPhiPQ} implies 
$E^{\mathrm{MAP}}(t_n)= \sum_{j=1}^n O(\epsilon_j^{\mathrm{MAP}})$.
%for the cubic MARS method with ARMS strategy.

The first step of estimating $\epsilon_j^{\mathrm{MAP}}$
is %the introduction of a semidiscrete flow map as follows.

\begin{defn}
  \label{def:semiDiscreteFlowMap}
  A \emph{semidiscrete flow map} is a function
  $\mathring{\phi}: \mathbb{Y} \rightarrow \mathbb{Y}$
  that results from discretizing the exact flow map $\phi$
  in time by a $\kappa$th-order ODE solver. 
  % $\mathring{\phi}_{t_0}^{nk}$ is \emph{$\kappa$th-order accurate}
  % up to time $T$ if
  % $\mathring{\phi}_{t_0}^{nk}(p)={\phi}_{t_0}^{nk}(p)+O(k^\kappa)$
  % for all $p(t_0)\in\mathbb{R}^2$ and $t_0+nk\le T$.
\end{defn}

Suppose a Runge-Kutta method is employed to discretize $\phi$. 
Then the semidiscrete flow map $\mathring{\phi}$
for the ODE (\ref{eq:velODE}) is of the form 
\begin{equation}
  \label{eq:semiDiscreteFlowMap}
   \mathring{\phi}_0^k(\mathbf{X}^0)
   := \mathbf{X}^0 + k \sum_{j=1}^{n_{\stage}} b_j \mathbf{y}_j
   \text{ where }
   \mathbf{y}_i = \mathbf{u}
   \left(\mathbf{X}^0 + k \sum\nolimits_{j=1}^{n_{\stage}} a_{ij} \mathbf{y}_j,
     t^0 + c_ik \right),
 \end{equation}
 where $a_{ij}$, $b_j$, $c_i$ constitute the standard Butcher tableau.

In the second step, we split $\epsilon_j^{\mathrm{MAP}}$ into 
% two error components, 
\begin{equation}
  \label{eq:keyMappingErrorItems}
  \renewcommand{\arraystretch}{1.5}
  \left\{
  \begin{array}{rl}
    \epsilon_j^{\textup{time}}
     & := \max_{\mathbf{X}\in\partial\mathcal{M}_\psi^{j-1}}
    \left\|\phi^k_{t_{j-1}}\mathbf{X}
    -\mathring{\phi}^k_{t_{j-1}}\mathbf{X}\right\|_2;        \\
    \epsilon_j^{\textup{space}}
     & := \max_{\mathbf{X}\in\partial\mathcal{M}_\psi^{j-1}}
    \left\|\mathring{\phi}^k_{t_{j-1}}\mathbf{X}
    -\varphi^k_{t_{j-1}}\mathbf{X}\right\|_2, 
  \end{array}
  \right.
\end{equation}
where $\epsilon_j^{\textup{time}}=O(k^{\kappa + 1})$
follows directly from Definition \ref{def:semiDiscreteFlowMap}
and the fact that $\mathring{\phi}$ acts
on \emph{all} points in $\partial\mathcal{M}_\psi^{j-1}$.

In the third step, we estimate $\epsilon_j^{\textup{space}}$ in
\begin{lem}
  \label{lem:accuracyOfDiscreteFlowMap}
  % Let $X_b$ be a $(r_{\Tiny}, h_L)$-regular
  %  breakpoint sequence and not-a-knot spline's breakpoint
  %  sequence satisfies $r_b < 1$.
  Suppose each piecewise smooth curve in $\partial \mathcal{M}_\psi^{j-1}$
  is approximated by a periodic or not-a-knot cubic spline
  as discussed in Sec.~\ref{sec:representation}. 
  % Consider the approximation of
  %  a semidiscrete flow map $\mathring{\phi}^k_{t_{j-1}}$ 
  %  with a discrete flow map
  %  ${\varphi^k_{t_{j-1}}}: \mathbb{Y} \rightarrow \mathbb{Y}$.
  % If $\mathring{\phi}^k_{t_{j-1}}$ is $\kappa$th-order accurate with $\kappa\ge 1$.
  %  Then, for each not-a-knot spline or periodic spline $p \in \mathbb{S}^{2}_3(X_b),\times \mathbb{S}^{2}_3(X_b) $, 
  %  which is used to represent 
  %  $\partial \mathcal{M}_\psi^{j-1}$,
  %  satisfies:
  Then %we have 
   \begin{equation}
     \label{eq:accuracyOfDiscreteFlowMap}
     \epsilon_j^{\textup{space}} =
     % \max_{p(x)\in\partial\mathcal{M}_\psi^{j-1}}
     % \left\|\mathring{\phi}^k_{t_{j-1}}p(x)
     % -\varphi^k_{t_{j-1}}p(x)\right\|_2
     % =
     O\left( k  h_{L}^4\right). 
   \end{equation}
   % When markers $\{\mathring{\phi}(p(x_{i}))\}$'s 
   % cumulative chordal length 
   % $\hat{X_b} := \{\hat{l}_i\}$ 
   % also satisfies $\hat{r}_b \ge 1$
   % for not-a-knot spline breakpoint sequences.
\end{lem}
\begin{proof}
  By (\ref{eq:keyMappingErrorItems}),
  $\epsilon_j^{\textup{space}} =
  \max_{p(x)\in\partial\mathcal{M}_\psi^{j-1}}
  \left\|\mathring{\phi}^k_{t_{j-1}}p(x)
    -\varphi^k_{t_{j-1}}p(x)\right\|_2$. 
  According to Definition \ref{def:semiDiscreteFlowMap},
  $\mathring{\phi}^k_{t_{j-1}}$ acts on all points in  
  $\partial \mathcal{M}_\psi^{j-1}$,
  and thus
  $\partial\left(\mathring{\phi}^k_{t_{j-1}}
    \mathcal{M}_\psi^{j-1}\right)$
  might not be a cubic spline.
  In contrast,
  we know from Definition \ref{def:ARMS}
  that $\varphi^k_{t_{j-1}}$ only acts on the markers of 
  $\partial \mathcal{M}_\psi^{j-1}$,
  the images of which are then used 
  to construct cubic splines.
  
  Denote by $l\in [l_0,l_{N}]$
  the corresponding cumulative chordal length 
  of the markers on $\partial\left(\mathring{\phi}^k_{t_{j-1}} \mathcal{M}_\psi^{j-1}\right)$
  and let $\mathbf{S}: [l_0,l_{N}]\rightarrow \mathbb{R}^2$
  be the spline fitted through these markers.
  Let $\mathbf{F}: [l_0,l_{N}]\rightarrow \mathbb{R}^2$
  be the functional form of the curve
  $\partial\left(\mathring{\phi}^k_{t_{j-1}}
    \mathcal{M}_\psi^{j-1}\right)$. 
  Then, we have
  \begin{displaymath}
   \begin{array}{l}
    \epsilon_j^{\textup{space}}
    % &=\max_{p(x)\in\partial\mathcal{M}_\psi^{j-1}}
    %  \left\|\mathring{\phi}^k_{t_{j-1}}p(x)
    %  -\varphi^k_{t_{j-1}}p(x)\right\| \\
    % &=
    %  \max_{{l}}
    %  \left\|\mathbf{F}_1(l)-\mathbf{S}_2(\tilde{l})\right\|_2\\
    =
    \max_{{l 
    \in [l_0,l_N]}}
    \left\|\mathbf{F}(l)-\mathbf{S}(l)\right\|_2 
    \leq c_0 h_L^{4}
    \max_{\xi\in[l_0,l_N]\setminus X_b}\left|
    \mathbf{F}^{(4)}(\xi)\right| 
    = O(kh_L^4).
   \end{array} 
  \end{displaymath}
   where the second step follows from 
   Theorems~\ref{thm:periodicSplineErrorEstimates} and 
   \ref{thm:notaKnotSplineErrorEstimates} 
   and the last from $\mathbf{F}^{(4)}(\xi)=O(k)$,
   an implication of Lemma \ref{lem:4thDerivIsOk}.  \qed
\end{proof}

\begin{lem}
  \label{lem:4thDerivIsOk}
  Let $\mathbf{p}: [0, \tilde{l}_{N}]\rightarrow\mathbb{R}^2$
  be a periodic or not-a-knot cubic spline
  fitted through a sequence
  $(\mathbf{X}^0_i)_{i=0}^{N}$ of breakpoints
  with $\tilde{l}_{i}$'s as the cumulative chordal lengths.
  Denote by $\Gamma(t)$ the loci of $\mathbf{p}$ at time $t\in[0,k]$
  under the action of a semidiscrete flow map $\mathring{\phi}$
  % on exact flow map $\mathbf{u}(x, t)$
  .
  Then we have
  \begin{equation}
    \label{eq:4thDerivIsOk}
    \forall \mathbf{X}\in \Gamma(k)\setminus
    \left\{\mathring{\phi}_0^k(\mathbf{X}^0_i):
     i=0,\ldots,N\right\}, 
    \quad
    \frac{\dif^4 \mathbf{X}(l)}{\dif l^4} = O(k), 
  \end{equation}
  where $l$ is the cumulative chordal length determined from
  the breakpoint sequence
  $(\mathbf{X}^k)$
  where $(\mathbf{X}^t):=
  \left(\mathring{\phi}_0^t(\mathbf{X}_i^0)\right)_{i=0}^{N}$.
\end{lem}
% \begin{proof} \revise{
%   See Sec.~\ref{sec:proof4thDerivIsOk} for the derivation.\qed }
% \end{proof}
\begin{proof}
  At any time $t\in[0,k]$,
  the curve $\Gamma(t)$ is parametrized by $l$,
  the cumulative chordal length of the sequence $(\mathbf{X}^t)$. 
  For any sufficiently small $k$,
  $\Gamma(t)(l)$ is homeomorphic
  to $\mathbf{p}(\tilde{l})$; in particular, $\Gamma(0)=\mathbf{p}$.
  Therefore, for any $t\in (0,k]$,
  there exists a bijective affine transformation
  that relates $l$ to $\tilde{l}$ and vice versa.
  Hence $\frac{\dif \tilde{l}}{\dif l}$ is a nonzero constant
  and $\frac{\dif^2 \tilde{l}}{\dif l^2}=0$.
  By (\ref{eq:semiDiscreteFlowMap}), we have
  \begin{equation}
    \label{eq:expansionOfXatX0}
    \begin{array}{l}
    \forall \mathbf{X}\in \Gamma(k),\ 
    \exists \mathbf{X}^0\in \mathbf{p}, \text{ s.t. }
    \mathbf{X} = \mathring{\phi}_0^k(\mathbf{X}^0)
    = \mathbf{X}^0 + k \sum_{j=1}^{n_{\stage}} b_j \mathbf{y}_j,
    \end{array}
  \end{equation}
  where $\mathbf{y}_i = \mathbf{u}
   \left(\mathbf{X}^0 + k \sum\nolimits_{j=1}^{n_{\stage}} a_{ij} \mathbf{y}_j,
     t^0 + c_ik \right)$. 
  The fourth derivative of (\ref{eq:expansionOfXatX0})
  %with respect to $l$
  at any $\mathbf{X}\not\in
        \left\{\mathring{\phi}_0^k(\mathbf{X}^0_i):
        i=0,\ldots,N\right\}$, 
      the chain rule, and $\frac{\dif^2 \tilde{l}}{\dif l^2}=0$ yield
  \begin{displaymath}
    \begin{array}{l}
    \frac{\dif^4 \mathbf{X}(l)}{\dif l^4}
    = \frac{\dif^4 \mathbf{X}^0}{\dif \tilde{l}^4}
    \left(\frac{\dif \tilde{l}}{\dif l}\right)^4
    + k \sum_{j=1}^{n_{\stage}} b_j \frac{\dif^4 \mathbf{u}}{\dif l^4}
    + O(k^2). 
    \end{array}
  \end{displaymath}
  Then the proof is completed by
  $\frac{\dif^4 \mathbf{X}^0}{\dif \tilde{l}^4}\equiv 0$, 
  i.e., the fourth derivative of any cubic polynomial vanishes.
   \qed 
\end{proof}

To sum up, we have, from (\ref{eq:individualerror}c), (\ref{eq:keyMappingError}),
 (\ref{eq:keyMappingErrorItems}),
 and Lemma \ref{lem:accuracyOfDiscreteFlowMap}, 
 \begin{equation}
   \label{eq:mappingError4thOrder}
   \begin{array}{l}
   E^{\mathrm{MAP}} \le \sum\nolimits_j \epsilon_j^{\mathrm{MAP}}
   = O\left(\frac{1}{k}\right) \left[
     O(k^{\kappa+1}) + O(k h_L^4)
   \right]
   = O(k^{\kappa}) + O(h_L^4).
   \end{array}
 \end{equation}
% \begin{proof}
% The Taylor expansion of $p$ over 
% each spatial interval $\left[x_i, x_{i+1}\right]$ 
% where $x_i \in X_b$ can be expressed as
% \begin{equation}
%   \label{eq:proveAcuracyOfDiscreteFlowMapTaylorU}
%   p(x) = p(x_i) + p'(x_i)(x-x_i) + \frac{p''(x_i)}{2}(x-x_i)^2 + \frac{p'''(x_i)}{6}(x-x_i)^3 + O(h_L^4),
% \end{equation}
% where the $O(h_L^4)$ term can be omitted since $p$ 
% is a cubic polynomial over $\left[x_i, x_{i+1}\right]$. 
% We define the Taylor approximation operator
% \begin{equation}
%   \mathcal{T}(p(x)) := p(x_i) + p'(x_i)(x-x_i) + \frac{p''(x_i)}{2}(x-x_i)^2 + \frac{p'''(x_i)}{6}(x-x_i)^3.
% \end{equation}

% By Definition \ref{def:splineFuncs}, 
% the values $p(x_i)$, $p'(x_i)$, $p''(x_i)$, and $p'''(x_i)$ 
% are uniquely determined
% by the set of breakpoints $P_b := \{p(x_i) \mid x_i \in X_b\}$. 
% From the definition of $\mathring{\phi}$, we obtain
% \begin{equation}
%   \label{eq:T_phi}
%   \begin{aligned}
%     \varphi_{t_n}^{k}(P_b)                     & = \mathring{\phi}_{t_n}^{k}(P_b)             \\
%     \implies \mathcal{T}(\varphi_{t_n}^{k}(p)) & = \mathcal{T}(\mathring{\phi}_{t_n}^{k}(p)).
%   \end{aligned}
% \end{equation}


% Let $\mathbf{u}$ denote the flow map on $\mathbb{R}^2$, 
% and define $\mathbf{u}^{(m)} := \frac{\partial^m \mathbf{u}}{\partial t^m}$
% for $m \geq 0$.
% The temporal Taylor expansion of $\phi_{t_n}^{k}(p(t_n))$ is given by
% \begin{equation}
%   \label{eq:flowMapTaylorExpansion}
%   \phi_{t_n}^{k}(p(t_n)) = p(t_n) + \sum_{i=0}^{\infty} \frac{k^{i+1}}{(i+1)!}
%   \left.
%   \frac{\partial^{i}\mathbf{u}(p(t_n+\tau), t_n+\tau)}{\partial \tau^{i}}
%   \right|_{\tau=0}.
% \end{equation}
% We define a linear combination as
% \begin{equation}
%   \label{eq:linearCombinationOfVelTimeDerivatives}
%   \begin{array}{rl}
%     \Delta^{(m)}_p := {\cal T} (\mathbf{u}^{(m)}(x)) (x, t)
%     - \mathbf{u}^{(m)}(x, t).
%   \end{array}
% \end{equation}
% For any fixed temporal instant, 
% the Taylor series expansion of $\mathbf{u}^{(m)}(x)$ about $x_i$ yields
% \begin{equation}
%   \label{eq:proveAcuracyOfDiscreteFlowMapTaylorUt}
%   \left\|\Delta^{(m)}_p \right\|
%   = O(h_L^4),
% \end{equation}
% where we have employed the result from equation
% (\ref{eq:proveAcuracyOfDiscreteFlowMapTaylorU}).
% Consequently, we derive the following error estimates:
% \begin{displaymath}
%   \renewcommand{\arraystretch}{1.4}
%   \begin{array}{rl}
%     \left\|{\varphi}_{t_n}^k(p)
%     - \mathring{\phi}_{t_n}^k(p)\right\|
%      & = \left\|{\cal T}(\mathring{\phi}_{t_n}^k(p))
%     - \mathring{\phi}_{t_n}^k(p) \right\|
%     \\
%      & = \left\| {\cal T}({\phi}_{t_n}^k(p))
%     - {\phi}_{t_n}^k(p) \right\|
%     + O(k^{\kappa+1})
%     \\
%      & =\left\| \sum_{i=0}^{\kappa-1} \frac{k^{i+1}}{(i+1)!} \Delta_p^{(i)} \right\|
%     + O(k^{\kappa+1})
%     \\
%      & = O(kh_L^4) + O(k^{\kappa+1}),
%   \end{array}
% \end{displaymath}
% where the first step follows from ${\varphi}_{t_n}^k(p)$
% is a cubic polynomial on interval $\left[x_i, x_{i+1}\right]$, 
% (\ref{eq:proveAcuracyOfDiscreteFlowMapTaylorU}) and (\ref{eq:T_phi}),
% the second step from
% the assumption of $\mathring{\phi}$ being
% $\kappa$th-order accurate,
% the third step from
% (\ref{eq:flowMapTaylorExpansion})
% and (\ref{eq:linearCombinationOfVelTimeDerivatives}),
% and the last step from
% (\ref{eq:proveAcuracyOfDiscreteFlowMapTaylorUt}).
% \end{proof}

% Finally, we present the principal conclusion of this subsection.
% \begin{lem}
%   \label{lem:EMAPbound}
%   The cubic MARS method with ARMS strategy
%   yields:
%   \begin{equation}
%     \label{eq:EMAPbound}
%     E^{\mathrm{MAP}}(t_n) = O(h_L^4) + O(k^\kappa),
%   \end{equation}
%   where $\kappa$ denotes the temporal discretization order.
% \end{lem}
% \begin{proof}
%   Following Lemma \ref{lem:accuracyOfDiscreteFlowMap}, 
%   the maximal deviation between corresponding points 
%   on the boundaries $\partial\phi^k_{t_{j-1}}\mathcal{M}_\psi^{j-1}$ 
%   and $\partial\varphi^k_{t_{j-1}}\mathcal{M}_\psi^{j-1}$ satisfies
%   \begin{equation}
%     \epsilon_j^{\mathrm{MAP}} \leq \epsilon_j^{\textup{time}} + \epsilon_j^{\textup{space}} 
%     = O(k^{\kappa+1}) + O(k h_L^4).
%   \end{equation}
%   The proof is then completed by
%   (\ref{eq:individualerror}c) and Lemma \ref{lem:normOfPhiPQ}.
% \end{proof}

\subsection{The adjustment error  $E^{\mathrm{ADJ}}$}
\label{sec:adjustmenterror}

\begin{figure}
  \centering
  \includestandalone[width=0.5\textwidth]{{\TIKZDIR}removingPointonSpline}
  \caption{The removal of a marker $p_i$
    from the breakpoint sequence $(p_i)_{i=0}^N$ of a cubic spline
    is equivalent to perturbing $p_i$ to $\hat{p}_i$
    on the new spline as the output of $\chi_{j}$, which, fitted through
    the new sequence $(p_0,p_1,\ldots,p_{i-1}, p_{i+1},\ldots, p_N)$,
    is ${\cal C}^3$ at $\hat{p}_i$.
  }
  \label{fig:removingpointonSpline}
\end{figure}

Consider a smooth curve $\partial\mathcal{M}_S^j$ 
 that interpolates all markers
 of $\partial\varphi_{t_{j-1}}^k\mathcal{M}_\psi^{j-1}$ 
 and $\partial\mathcal{M}^j$,  
 %which, according to (\ref{eq:individualerror}d),
 the cubic splines immediately 
 before and after performing the adjustment operation 
 \ref{en:arms-remove}, respectively.
Both splines can be considered as approximations
 of the smooth curve $\partial\mathcal{M}_S^j$. 
By Theorems~\ref{thm:periodicSplineErrorEstimates} and 
 \ref{thm:notaKnotSplineErrorEstimates},
 the distance between corresponding points
 is ${O}(h_L^4)$. 
Therefore, removing a marker can be regarded as 
 performing an $O(h_L^4)$ perturbation to that point and 
 reconstructing the spline; see Fig.~\ref{fig:removingpointonSpline}.
For any sufficiently small $k>0$,
 the marker sequence of
 $\partial\varphi_{t_{j-1}}^k\mathcal{M}_\psi^{j-1}$
 satisfies the $(r,h_L)$-regularity for some
 $r\in (0,r_{\Tiny}]$. 
Then Lemma \ref{lem:splineLocality},
 Lemma~\ref{lem:normOfPhiPQ},
 and the fact of the error over $[l_{i-1},l_{i+1}]$ 
 around the perturbed marker $p_i$ being
 $O(h_L)\cdot O(h_L^4) = O(h_L^5)$ imply
\begin{equation}
  \label{eq:adjustmentErrorOneStep}
  \left\|\phi_{t_j}^{(n-j)k}
  [\varphi_{t_{j-1}}^k\mathcal{M}_\psi^{j-1}, 
  \mathcal{M}^j]\right\| 
  = N_r^{j-1}\cdot{O}(h_L^5),
\end{equation}
 where $N_r^j$ denotes the number of 
 removed markers within $[t_j,t_{j+1}]$. 
%
 Although it's difficult to control $N_r^j$ at each time step,
 we will prove in Lemma \ref{lem:numberRemovedMarkers}
 that the total number of removed markers 
 during the entire IT in $[0,T]$
 is $O\left(\frac{1}{h_L}\right)$, i.e.,
 $N_r := \sum\nolimits_{j=0}^{\frac{T}{k}-1} N_r^j
  = O\left(\frac{1}{h_L}\right)$,
which, together with (\ref{eq:adjustmentErrorOneStep})
and (\ref{eq:individualerror}d), 
implies
% $E^{\mathrm{ADJ}}(T)=O(h_L^4)$.
% By (\ref{eq:adjustmentErrorOneStep}) and 
% Lemma \ref{lem:numberRemovedMarkers}, the adjustment error accumulates as
\begin{equation}
  \label{eq:EADJbound}
  E^{\mathrm{ADJ}}(t_n) = \left\Vert\bigoplus_{j=1}^{n}
    \phi_{t_j}^{(n-j)k}[\varphi_{t_{j-1}}^k\mathcal{M}_\psi^{j-1},
    \mathcal{M}^j] \right\Vert
  = {O}\left(\frac{1}{h_L}\right)\cdot{O}(h_L^5) = {O}(h_L^4).
\end{equation}

We start our journey to Lemma \ref{lem:numberRemovedMarkers}
by examining how the discrete flow map changes
the distance between adjacent markers.

\begin{lem}
  \label{lem:discreteFlowMapOnChordalLength}
  The discrete flow map 
  $\varphi_{t_n}^k: \mathbb{Y}\to \mathbb{Y}$
  in Definition \ref{def:MARS} satisfies
  \begin{equation}
    \label{eq:discreteFlowMapOnChordalLength}
    \|p_{i+1} - p_{i}\|_2 - \|X_{i+1} - X_{i}\|_2 = O(k h_L), 
  \end{equation}
  where $X_{i+1},X_{i}$ are two adjacent markers
  and $p_i := \varphi_{t_n}^k(X_i)$ the image of $X_i$.
\end{lem}
% \begin{proof}\revise{
%   See Sec.~\ref{sec:proofdiscreteFlowMapOnChordalLength} for the derivation.\qed }
% \end{proof}
\begin{proof}
  By (\ref{eq:semiDiscreteFlowMap}), we have
   \begin{equation*}
     p_i = X_i + k \sum\nolimits_{j=1}^{n_{\stage}} b_j \mathbf{y}_{i,j}
    \text{ where }
    \mathbf{y}_{i,j} = \mathbf{u}
    \left(X_i + k \sum\nolimits_{l=1}^{n_{\stage}} a_{jl} \mathbf{y}_{i,l},
      t_n + c_j k \right), 
   \end{equation*}
   which yields the Lipschitz estimate
  \begin{eqnarray*}
    \begin{aligned}
    \left\|\mathbf{y}_{i+1,j} - \mathbf{y}_{i,j} \right\|_2
    \le & L \left\|X_{i+1} - X_{i} + 
    k \sum\nolimits_{l=1}^{n_{\stage}} a_{jl} 
    (\mathbf{y}_{i+1,l} -\mathbf{y}_{i,l})\right\|_2 \\
    \le & L \left(\left\|X_{i+1} - X_{i} \right\|_2 + 
    k \sum\nolimits_{l=1}^{n_{\stage}} |a_{jl}| 
    \left\|\mathbf{y}_{i+1,l} -\mathbf{y}_{i,l} \right\|_2\right) \\
    \le & L \left(\left\|X_{i+1} - X_{i} \right\|_2 + 
     a_{\max} k\sum\nolimits_{l=1}^{n_{\stage}} 
     \left\|\mathbf{y}_{i+1,l} -\mathbf{y}_{i,l} \right\|_2\right),
    \end{aligned}
  \end{eqnarray*}
   where $L$ is the Lipschitz constant of $\mathbf{u}$
   and $a_{\max} := \max|a_{jl}|$.
  Sum both sides of the above inequality for $j=1,2,\ldots,n_{\stage}$
   and we obtain
  \begin{small}
  \begin{eqnarray*}
    \begin{aligned}
     & \sum\nolimits_{j=1}^{n_{\stage}}
     \left\|\mathbf{y}_{i+1,j} - \mathbf{y}_{i,j} \right\|_2
     \le Ln_{\stage} \left( \left\|X_{i+1} - X_{i} \right\|_2 + 
     a_{\max} k\sum\nolimits_{l=1}^{n_{\stage}} 
     \left\|\mathbf{y}_{i+1,l} -\mathbf{y}_{i,l} \right\|_2\right)\\
     \implies & \sum\nolimits_{j=1}^{n_{\stage}}
     \left\|\mathbf{y}_{i+1,j} - \mathbf{y}_{i,j} \right\|_2
     \le \frac{Ln_{\stage}}{1-Ln_{\stage}a_{\max} k} 
     \left\|X_{i+1} - X_{i} \right\|_2 = O(h_L)
    \end{aligned}
  \end{eqnarray*}
  \end{small}
  where $Ln_{\stage}a_{\max} k < 1$ for a sufficiently small $k$.
  The proof is completed by %rest follows from 
  \begin{align*}
    % \begin{aligned}
    & \left\|p_{i+1} - p_{i} \right\|_2 - 
      \left\|X_{i+1} - X_{i} \right\|_2 \\
    = & \left\| X_{i+1} - X_{i} + k\sum\nolimits_{j=1}^{n_{\stage}}
        b_j \left(\mathbf{y}_{i+1,j} - \mathbf{y}_{i,j} \right)
        \right\|_2 - \left\|X_{i+1} - X_{i} \right\|_2 \\
    \le &\ k\sum\nolimits_{j=1}^{n_{\stage}}
          |b_j| \left\|\mathbf{y}_{i+1,j} - \mathbf{y}_{i,j} \right\|_2 
    \le \ k \left\| \mathbf{b} \right\|_{\infty}
          \sum\nolimits_{j=1}^{n_{\stage}}
          \left\|\mathbf{y}_{i+1,j} - \mathbf{y}_{i,j} \right\|_2\\
    = &\ O(kh_L). \hspace{9cm} \qed
  % \end{aligned} 
  \end{align*} 
\end{proof}

Next, define the \emph{total $\mu$-variation
 of a marker sequence} $X_b = (X_i)_{i=0}^{N}$ as
\begin{equation}
  \label{eq:totalVariation}
  V(X_b) := \sum\nolimits_{i=0}^{N-1}\bigl|\left\|X_{i+1} - X_{i} 
  \right\|_2 - \mu h_L \bigr|,
\end{equation}
where $\mu \in (2r_{\Tiny},\frac{1}{2}-r_{\Tiny})$.
Since $2 r_{\Tiny}<\frac{1}{2}-r_{\Tiny}$ implies $r_{\Tiny}< \frac{1}{6}$
and $r_{\Tiny}\to \frac{1}{6}$ yields $\mu \to \frac{1}{3}$, 
 hereafter we set $\mu = \frac{1}{3}$. 
% Hereafter $\mu = \frac{1}{3}$ is used throughout this work.
%  the supremum of the interval
%  $(2r_{\Tiny},\frac{1}{2}-r_{\Tiny})$ for $r_{\Tiny}=\frac{1}{6}$
As $V(X_b)\to 0$, % approaches zero,
 the distance between adjacent markers in $X_b$
 approaches a uniform distribution at $\mu h_L$.

\begin{lem}
  \label{lem:propertyTotalVariation}
  Consider the ARMS strategy in Definition~\ref{def:ARMS}
  with a periodic or not-a-knot cubic spline $\mathbf{s}^n$
  of which the breakpoint sequence $X_b^{n} := (X_i)_{i=0}^{N^n}$
  is $(r_{\Tiny},h_L)$-regular with 
  $r_b^{\ast}\in(1,\frac{1}{2r_{\Tiny}})$ and 
  $r_{\Tiny} \in 
  \left(0,  \min(\frac{1}{6}, \frac{1}{2r_b^{\ast}})\right)$.
  Let $X_b^{n+1}$ be the marker sequence of $\mathbf{s}^{n+1}$
  generated by the ARMS strategy. 
  Then for 
  the augmentation operation $\psi_n$,
  the discrete flow map $\varphi_{t_n}^k$,
  and the adjustment operation $\chi_{n+1}$
  in Definition~\ref{def:MARS}, we have 
   \begin{enumerate}[label=(\alph*)]
    \item the total $\mu$-variation is bounded both at $t_n$ and $t_{n+1}$, i.e.,
    \begin{equation*}
      V(X_b^n) = O(1), \ V(X_b^{n+1}) = O(1);
    \end{equation*}
    \item adding a marker in $\psi_n$ reduces the total $\mu$-variation 
     by $\mu h_L + O({h_L^2})$, i.e., %or equivalently,
    \begin{equation*}
      V(\psi_n(X_b^n)) - V(X_b^n) = N_a^n \cdot \left[
        -\mu h_L + O({h_L^2})\right],
    \end{equation*}
     where $N_a^n$ denotes the number of added markers
     at $t_n$;
    \item the discrete flow map $\varphi_{t_n}^k$ satisfies
    \begin{equation*}
      \left| \Delta V_{\varphi}^{n} \right| := 
      \left|V(\varphi_{t_n}^k \circ \psi_n(X_b^n)) - V(\psi_n(X_b^n)) \right| 
      = O(k);
    \end{equation*}
    \item removing markers in $\chi_{n+1}$
     strictly decreases the total $\mu$-variation, i.e.,
    \begin{equation*}
      V(X_b^{n+1}) 
      - V(\varphi_{t_n}^k \circ \psi_n(X_b^n)) = 
      V(\chi_{n+1}\circ \varphi_{t_n}^k \circ \psi_n(X_b^n)) 
      - V(\varphi_{t_n}^k \circ \psi_n(X_b^n)) 
      < 0.
    \end{equation*}
  \end{enumerate}
\end{lem}
% \begin{proof}\revise{
%   See Sec.~\ref{sec:proofpropertyTotalVariation} for the derivation.\qed }
% \end{proof}
\begin{proof}
  For (a), $\phi$ being a diffeomorphic flow map implies that 
  the total arc length of the cubic spline at any $t_n\in[0,T]$
  is $O(1)$. 
  Hence the number of markers is 
  \begin{equation}
    \label{eq:Nj}
    N^n \le \frac{L_{\partial \mathcal{M}^n}}
    {r_{\Tiny}h_L} = O\left(\frac{1}{h_L}\right),
  \end{equation}
  % \begin{equation}
  %   \label{eq:Nj}
  %   N_j = \frac{O(1)}{O(h_L)}
  %   = O\left(\frac{1}{h_L}\right),
  % \end{equation}
   where the inequality follows from the 
   $(r_{\Tiny},h_L)$-regularity of the sequence $X_b^n$.
  Consequently, we derive the bound 
  \begin{equation*}
    % \label{eq:totalVariationbounded}
    V(X_b^n) = \sum\nolimits_{i=0}^{N^{n}-1}\left|\left\|X_{i+1} - X_{i} 
    \right\|_2 - \mu h_L \right|
    \le N^n \cdot (1-\mu) h_L = O(1).
  \end{equation*}
  By Lemma~\ref{lem:rhRegularity},
  $X_b^{n+1}$ is also $(r_{\Tiny},h_L)$-regular
  and thus $V(X_b^{n+1}) = O(1)$ follows
  from similar arguments.

  For (b),  
  Lemma~\ref{lem:discreteFlowMapOnChordalLength} implies
  that only one marker, say $X$,
  is added between $X_i$ and $X_{i+1}$
  for any sufficiently small $k>0$.
  Then \ref{en:arms-add} 
   and the form of cubic splines in (\ref{eq:SForm2}) imply
  \begin{eqnarray}
    \begin{aligned}
      \label{eq:adjacentX}
      \left\| X_{i+1} - X \right\|_2
      & = \frac{1}{2} \left\| X_{i+1}
      - X_i \right\|_2 + O(h_L^2),\\
      \left\| X - X_{i} \right\|_2
      & = \frac{1}{2} \left\| X_{i+1}
      - X_i \right\|_2 + O(h_L^2).
    \end{aligned}
  \end{eqnarray}
  For the augmentation operation $\psi_n^{(1)}$ 
   that adds a single marker $X$ between $X_i$ and $X_{i+1}$, 
   we claim 
  \begin{equation}
    \label{eq:totalVariationpsi}
    \Delta V_{\psi}^{(1)}
      := V(\psi_n^{(1)}(X_b^n)) - V(X_b^n)
      = - \mu h_L + O(h_L^2).
  \end{equation} 
  Indeed,
  $h_L^{\ast} = (1-2r_{\Tiny})h_L$
  in \ref{en:arms-add}, 
  $r_{\Tiny}<\frac{1}{6}$, and $\mu=\frac{1}{3}$
  gives \mbox{$h_L^{\ast}>2\mu h_L$}. 
  As $k\to 0$, 
  (\ref{eq:discreteFlowMapOnChordalLength})
  and % the condition
  $\left\|p_{i+1}-p_i\right\| > h_L^{\ast}$ in \ref{en:arms-add}
  yield 
  \begin{equation*}
    \left\| X_{i+1} - X_i \right\|_2
    = \left\| p_{i+1} - p_i \right\|_2 + O(kh_L) 
    > h_L^{\ast} + O(kh_L) > 2\mu h_L, 
  \end{equation*}
  which, together with (\ref{eq:adjacentX}), implies 
  \begin{eqnarray*}
    \begin{aligned}
      \Delta V_{\psi}^{(1)} 
%       = & V(\psi_n^{(1)}(X_b^n)) - V(X_b^n) \\
       = & \left| \left\|X_{i+1} - X \right\|_2 - \mu h_L\right|
       + \left| \left\|X - X_{i} \right\|_2 - \mu h_L\right| 
       - \left| \left\|X_{i+1} - X_{i}\right\|_2 - \mu h_L\right|
        \\
      = & 2\left|\frac{1}{2} \left\| X_{i+1} - X_i \right\|_2 
      + O(h_L^2) - \mu h_L\right|
      - \left| \left\|X_{i+1} - X_{i} \right\|_2 - \mu h_L\right|\\
      = & \left\|X_{i+1} - X_{i} \right\|_2 - 2\mu h_L 
      - \left(\left\| X_{i+1} - X_i \right\|_2 - \mu h_L \right)  + O(h_L^2)\\
      = & - \mu h_L + O(h_L^2).
    \end{aligned}
  \end{eqnarray*}
  Then (b) follows from summing up $\Delta V_{\psi}^{(1)}$
  for the $N_a^n$ added markers.
  
  (c) holds because
  \begin{eqnarray*}
    \begin{aligned}
      %\label{eq:totalVariationvarphi}
      \left| \Delta V_{\varphi}^{n} \right|
      % = & \left|V(\varphi_{t_n}^k \circ \psi_n(X_b^n)) 
      % - V(\psi_n(X_b^n)) \right|\\
      = & \sum\nolimits_{i=0}^{N^n + N_a^n -1}\left(
        \left|\left\|p_{i+1} - p_{i} 
    \right\|_2 - \mu h_L \right| - 
    \left|\left\|X_{i+1} - X_{i} 
    \right\|_2 - \mu h_L \right|
      \right)\\
      \le & \sum\nolimits_{i=0}^{N^n + N_a^n -1}  
      \left| \left\|p_{i+1} - p_{i} \right\|_2 - \mu h_L -
             \left\|X_{i+1} - X_{i} \right\|_2 + \mu h_L\right|\\
      = & \sum\nolimits_{i=0}^{N^n + N_a^n -1} O(kh_L) \\
      = & \ O(k),
    \end{aligned}
  \end{eqnarray*}
   where the third step follows from %penultimate
   (\ref{eq:discreteFlowMapOnChordalLength}) 
   and the last from (\ref{eq:Nj})
   and $N_a^n \le N^n$ for any sufficiently small $k>0$.

   For (d), consider three consecutive markers $p_i$, $p_{i+1}$, and $p_{i+2}$
   that satisfy
   \begin{displaymath}
     \|p_{i+1} - p_{i}\|_2 = ah_L< r_{\Tiny} h_L;\quad
     \|p_{i+2} - p_{i+1}\|_2 = bh_L > 0.
   \end{displaymath}
  For the adjustment operation $\chi_{n+1}^{(1)}$
   that removes the marker $p_{i+1}$, 
   we have 
  \begin{equation}
    \label{eq:totalVariationchi}
    \Delta V_{\chi}^{(1)} 
      := V(\chi_{n+1}^{(1)} \circ \varphi_{t_n}^k \circ \psi_n(X_b^n)) 
      - V(\varphi_{t_n}^k \circ \psi_n(X_b^n)) < 0,
  \end{equation} 
   because
  \begin{eqnarray*}
    \begin{aligned}
      \Delta V_{\chi}^{(1)} 
      % =&V(\chi_{n+1}^{(1)} \circ \varphi_{t_n}^k \circ \psi_n(X_b^n)) 
      % - V(\varphi_{t_n}^k \circ \psi_n(X_b^n)) \\
      =& 
      \left| \left\|p_{i+2} - p_{i} \right\|_2 - \mu h_L \right| -
      \left| \left\|p_{i+2} - p_{i+1} \right\|_2 - \mu h_L\right| -
      \left| \left\|p_{i+1} - p_{i} \right\|_2 - \mu h_L\right| \\
      =& \left(\left|a+b+O(h_L) - \mu \right| - 
      \left|b - \mu\right| - 
      \left|a - \mu\right| \right)h_L \\
      =& \begin{cases}
       \max\left(2(a+b) - 3\mu + O(h_L), -\mu + O(h_L)\right)h_L & \text{if}\ b 
       \le \mu;\\
        \left(2a - \mu +O(h_L)\right)h_L 
        & \text{if}\ b > \mu
      \end{cases}\\
     <&\ 0,
    \end{aligned}
  \end{eqnarray*}
   where the second step follows from the second-order accuracy
   of approximating the interface with linear segments
   and the last from $2a< 2r_{\Tiny} < \mu =\frac{1}{3}$.
%   $2a< 2r_{\Tiny}h_L < \mu h_L < \frac{1}{2}h_L^{\ast}$,
   % where $h_L^{\ast} = (1-2r_{\Tiny})h_L$ is defined in 
   % \ref{en:arms-add}.
  % The condition $r_{\Tiny} < \frac{1}{6}$ implies
  %  $2a < 2r_{\Tiny} < \mu$ in (\ref{eq:muRelation}).
  Then (d) follows from summing up $\Delta V_{\chi}^{(1)}$
   for the $N_r^n$ removed markers. \qed
\end{proof}

We are now ready to state and prove the following key result of this subsection.

\begin{lem}
  \label{lem:numberRemovedMarkers}
  Suppose that the preconditions of
  the ARMS strategy in Definition~\ref{def:ARMS} hold.
  Then the total number of removed markers
  during the entire IT in $[0,T]$
  by the multiphase MARS method in Definition~\ref{def:MARS-for-multiple-phases}
  is $O\left(\frac{1}{h_L}\right)$, i.e., 
  \begin{equation}
    \label{eq:numberRemovedMarkers}
    \forall T > 0,\quad N_r = \sum_{j=0}^{\frac{T}{k}-1} N_r^j
    = O\left(\frac{1}{h_L}\right).
  \end{equation}
\end{lem}
% \begin{proof}\revise{
%   See Sec.~\ref{sec:proofnumberRemovedMarkers} for the derivation.\qed }
% \end{proof}
\begin{proof}
  Since any Yin set is semianalytic,
  its boundary can be represented by a finite number of curves, 
  hence it suffices to prove (\ref{eq:numberRemovedMarkers})
  for a single spline.
  The only ways to change the total $\mu$-variation in (\ref{eq:totalVariation})
   are through the augmentation operation, 
   the fully discrete mapping operation, 
   and the adjustment operation that constitute a MARS method. 
  Denote by $N_a$ and $N_r$
   the total numbers of added and removed markers, respectively.
  The total $\mu$-variation change is 
  \begin{equation*}
    \Delta V  = V(X_b^{\frac{T}{k}}) - V(X_b^0) = 
    \sum\nolimits_{j=0}^{\frac{T}{k}-1}\Delta V_{\varphi}^{j}
    + \sum\nolimits_{i=1}^{N_a} \Delta V_{\psi,i}^{(1)}
    + \sum\nolimits_{i=1}^{N_r}\Delta V_{\chi,i}^{(1)},
  \end{equation*}
  where the subscript $_i$ indicates an added or removed marker.
  Then we have 
  \begin{eqnarray*}
    \begin{aligned}
      \left|\sum\nolimits_{i=1}^{N_a} \Delta V_{\psi,i}^{(1)}\right|
      &= - \sum\nolimits_{i=1}^{N_a} \Delta V_{\psi,i}^{(1)} 
      = -\Delta V + 
      \sum\nolimits_{j=0}^{\frac{T}{k}-1}\Delta V_{\varphi}^{j} 
      + \sum\nolimits_{i=1}^{N_r}\Delta V_{\chi,i}^{(1)}
      \\
      &< -\Delta V + \sum\nolimits_{j=0}^{\frac{T}{k}-1}\Delta V_{\varphi}^{j}
      = O(1) + O\left(\frac{1}{k}\right)\cdot O(k) = O(1).
    \end{aligned}
  \end{eqnarray*}
   where the first step follows from (\ref{eq:totalVariationpsi}),
   the third from (\ref{eq:totalVariationchi}),
   and the fourth from Lemma~\ref{lem:propertyTotalVariation}(a,c).
  Finally, combining (\ref{eq:Nj}) with 
   $\left|\Delta V_{\psi,i}^{(1)}\right| = \mu h_L + O(h_L^2)$ in 
   (\ref{eq:totalVariationpsi}), we get
   $N_a = O\left(\frac{1}{h_L}\right)$ and
   $N_r = N_a + N^0 - N^{\frac{T}{k}} = O\left(\frac{1}{h_L}\right)$. \qed
\end{proof}

The rest of this subsection is a proof of existence
 of the smooth curve $\partial\mathcal{M}_S^j$
 mentioned at the beginning of this subsection.

A set of $\mathcal{C}^\infty$ functions
 $\{\rho_\alpha: M\to [0, +\infty)\}_{\alpha\in I_{\alpha}}$
 defined on a manifold $M$ is called
 a \emph{$\mathcal{C}^\infty$ partition of unity} 
 if $\sum_{\alpha\in I_{\alpha}}\rho_\alpha=1$
 and the corresponding set of supports,
 written $\{\text{supp }\rho_\alpha\}_{\alpha\in I_{\alpha}}$,
 is locally finite, i.e.,
 any point \mbox{$x\in M$} has a local neighborhood that meets only
 a finite number of supports in
 $\{\text{supp }\rho_\alpha\}_{\alpha\in I_{\alpha}}$. 

\begin{thm}[Existence of a $\mathcal{C}^\infty$ partition of unity {\cite[Theorem 13.7]{Tu2011}}]
  \label{thm:ExistencePartitionOfUnity}
  For any open cover $\{U_\alpha \}_{\alpha\in I_{\alpha}}$ of a manifold $M$, 
  there exists a $\mathcal{C}^\infty$ partition of unity
  $\{\rho_\alpha\}_{\alpha\in I_{\alpha}}$ on $M$
  such that 
  $\text{supp }\rho_\alpha\subset U_\alpha$ for every $\alpha\in I_{\alpha}$.
\end{thm}
% \begin{proof}
%   See \cite[Theorem 13.7]{Tu2011}. 
% \end{proof}

\begin{lem}
  \label{lem:siErrSplineSmoothCurve}
  For any periodic or not-a-knot spline
  $\mathbf{p}: [l_0,l_{N}]\rightarrow \mathbb{R}^2$
  with its cumulative chordal lengths as $(l_i)_{i=0}^N$,
  there exists a smooth curve $\gamma\in {\cal C}^{\infty}$
  such that $\mathbf{p}(l_i)\in \gamma$
  for each $i=0,\ldots, N$.
\end{lem}
% \begin{proof}\revise{
%   See Sec.~\ref{sec:proofsiErrSplineSmoothCurve} for the derivation.\qed }
% \end{proof}
\begin{proof}
  For any positive real number $\epsilon <\frac{1}{4}\min_{i=1}^{N} |l_{i}-l_{i-1}|$,
  the 1-manifold $I_{\mathbf{p}}:=(l_0-\epsilon, l_{N}+\epsilon)$
  has an open cover $(U_j)_{j=0}^{2N}$ given by 
  \begin{equation}
    \label{eq:openCoverOfDomain}
    U_j :=
    \begin{cases}
      \left(l_{\frac{j}{2}}-2\epsilon,\
        l_{\frac{j}{2}}+2\epsilon\right)
      & \text{ if $j$ is even};
      \\
      \left(l_{\frac{j-1}{2}}+\epsilon,\ l_{\frac{j-1}{2}+1}-\epsilon\right)
      & \text{ if $j$ is odd}.
    \end{cases}
  \end{equation}

  Theorem \ref{thm:ExistencePartitionOfUnity} implies the existence
  of a partition of unity $(\rho_j)_{j=0}^{2N}$ satisfying
  $\text{supp }\rho_j\subset U_j$ and
  $\sum_{j=0}^{2N}\rho_j\equiv1$ on $I_{\mathbf{p}}$,
  which, together with (\ref{eq:openCoverOfDomain}), further yield
  \begin{displaymath}
    \left\{
      \begin{array}{lll}
        \forall i=0,\ldots, N,\ 
        &\forall l\in (l_i-\epsilon, l_i+\epsilon), \quad
        &\rho_{2i}(l) = 1;
        \\
        \forall i=0,\ldots, N-1,\ 
        &\forall l\in (l_i+2\epsilon, l_{i+1}-2\epsilon), \quad
        &\rho_{2i+1}(l) = 1.
      \end{array}
    \right.
  \end{displaymath}
  
  For each $i=0,\ldots,N-1$,
  we construct %a pair of quadratic polynomials
  $\mathbf{q}_i\in \mathbb{P}_{2} \times\mathbb{P}_2 $
  over $(l_i-2\epsilon, l_i+2\epsilon)$
  by requiring
  $\mathbf{q}_i(l_i)=\mathbf{p}(l_i)$
  and $\frac{\dif^2 \mathbf{q}_i}{\dif s^2}(l_i)
  =\frac{\dif^2 \mathbf{p}}{\dif s^2}(l_i)$. 
  For a periodic spline,
  we also set $\mathbf{q}_{N}(l):=\mathbf{q}_1(l-l_{N})$.
  % \begin{displaymath}
  %   \forall i=1,\ldots, N,\quad  \mathbf{p}_i(l)\in \mathbb{P}_m (U)\times\mathbb{P}_m (U),  \quad \mathbf{p}_i|_{[l_i,l_{i+1}]}=\mathbf{p}|_{[l_i,l_{i+1}]}, \quad 
  %   \mathbf{p}_0(l)=p_N(l+b-a),\quad
  %   \mathbf{p}_{N+1}(l)=\mathbf{p}_1(l-b+a).
  % \end{displaymath}
    
 Now we define a curve $\gamma: I_{\mathbf{p}}\to \mathbb{R}^2$ by
  \begin{equation}
    \label{eq:constructedSmoothCurve}
    \gamma(l):= \sum_{i=0}^{N} \rho_{2i}(l) \mathbf{q}_i(l)
    +\sum_{i=0}^{N-1} \rho_{2i+1}(l) \mathbf{p}_i(l),    
  \end{equation}
 where $\mathbf{p}_i:= \left.\mathbf{p}\right|_{(l_i, l_{i+1})}$
 is the pair of polynomials of $\mathbf{p}$ on the $i$th interval.
By the above construction,     
$\gamma$ is in ${\cal C}^{\infty}$. 
In particular, a periodic spline satisfies 
\begin{displaymath}
 \gamma^{(j)}(l_{N})
  =\left[
    \rho_{2N}(l_{N}) \mathbf{q}_{N}(l_{N})\right]^{(j)}
  = \mathbf{q}_{N}^{(j)}(l_{N})
  = \mathbf{q}_{0}^{(j)}(0)
  =\left[
    \rho_{0}(l_{0}) \mathbf{q}_{0}(l_{0})\right]^{(j)}
  =\gamma^{(j)}(l_0) 
\end{displaymath}
for any nonnegative integer $j$.  \qed
\end{proof}


\subsection{Convergence of the multiphase cubic MARS method}
\label{sec:IT_accuracy}

The main result of this section is 
\begin{thm}
  \label{thm:ITerrorOfMultiMARS}
  Suppose in Definition \ref{def:MARS-for-multiple-phases} that
  \begin{itemize}
  \item the discrete flow map $\varphi_{t_n}^k$
    is $\kappa$th-order accuracy in approximating
    the homeomorphic flow map $\phi$,
  \item all junctions and ${\cal C}^4$ discontinuities of the initial interface
    $\Gamma^0$ are contained in the vertex set of the interface graph, 
  \item the marker sequence of each fitted spline in $S_{CT}^0$
    is $(r_{\Tiny}, h_L)$-regular
    with $r_b^{\ast}\in(1,\frac{1}{2r_{\Tiny}})$
    and $r_{\Tiny} \in \left(0,  \min(\frac{1}{6},
      \frac{1}{2r_b^{\ast}})\right)$.
  \end{itemize}
  Then the multiphase MARS method
  in Definition \ref{def:MARS-for-multiple-phases}
  is convergent for solving the multiphase IT problem
  in Definition \ref{def:interfaceTracking}
  and its solution error satisfies
  \begin{equation}
    \label{eq:IT_error}
    \forall T>t_0,\quad E_{\mathrm{IT}}(T)  = {O}(h_L^4) + {O}(k^\kappa).
  \end{equation}
\end{thm}
\begin{proof}\revise{
  (\ref{eq:IT_error}) follows from 
  (\ref{eq:EREPbound}), (\ref{eq:EAUGbound}),
  (\ref{eq:mappingError4thOrder}), (\ref{eq:EADJbound}),
  and Theorem \ref{thm:errorsplit}.
  The convergence of the MARS method follows
  from that of the discrete flow map. %employed time integrator.
   \qed }
\end{proof}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../MARS-n2D"
%%% End:

% LocalWords:  multiphase semidiscrete affine bijective homeomorphic
% LocalWords:  nonnegative


==> tab/figure4-1c.tex <==
\scriptsize	
\begin{tabular}{c|c|c|c|c|c}
  \hline
  % a connected Yin set
  $\mathcal{M}_{i,j}$
  & %oriented Jordan curves in
    $\gamma_{i,j}^k$
  & directed cycle $C^k_{i,j}$ of $\gamma^k_{i,j}$
  & smooth?
  & $\mathbf{e}\in C_S$
  & $\mathbf{e}\in T_S$
  \\ \hline
  \multirow{1}{*}{$\mathcal{M}_1$}&$\gamma_1^{+}$
  & $e_2 \rightarrow e_3 \rightarrow e_5$ 
  & no
  & - & $(e_5)$
  \\ \hline
  \multirow{1}{*}{$\mathcal{M}_2$}&$\gamma_2^{+}$
  & $e_5 \rightarrow e_6 \rightarrow e_7$
  & no
  & - & $(e_5)$
  \\ \hline
  \multirow{1}{*}{$\mathcal{M}_3$}&$\gamma_3^{+}$
  & $e_3 \rightarrow e_4 \rightarrow e_6$
  & no 
  & - & $(e_3, e_6)$
  \\ \hline
  \multirow{3}{*}{$\mathcal{M}_{4,1}$}&$\gamma_{4,1}^{+}$
  & $e_1 \rightarrow e_9$ {\footnotesize (counterclockwise)}
  & yes
  & $(e_1,e_9)$ & -
  \\ & $\gamma_{4,1}^{1-}$
  & $e_2 \rightarrow e_7 \rightarrow e_{4}$
  & yes 
  & $(e_2, e_7, e_{4})$ & -
  \\ & $\gamma_{4,1}^{2-}$
  & $e_8$  {\footnotesize (clockwise)} 
  & yes 
  & $(e_8)$ & -
  \\ \hline
  \multirow{1}{*}{$\mathcal{M}_{4,2}$} & $\gamma_{4,2}^{+}$
  & $e_{13} \rightarrow e_{12} \rightarrow e_{14}$
  & no 
  & - & {\small $(e_{13}, e_{12}, e_{14})$}
  \\ \hline
  \multirow{3}{*}{$\mathcal{M}_{5}$} 
  & $\gamma_{5}^{+}$
  & $e_9 \rightarrow e_{12}$ {\footnotesize (counterclockwise)}
  & no 
  & - & -
  \\
  & $\gamma_{5}^{1-}$
  & $e_{10} \rightarrow e_{15}$  {\footnotesize (clockwise)}
  & no 
  & - & $(e_{15}, e_{10}, e_{11}, e_{16})$ 
  \\
  & $\gamma_{5}^{2-}$
  & $e_{16} \rightarrow e_{11}$  {\footnotesize (clockwise)}
  & no 
  & - & $(e_{15}, e_{10}, e_{11}, e_{16})$ 
  % \\ \hline
  % \multirow{1}{*}{$\mathcal{M}_{5,2}$} & $\gamma_{5,2}^{+}$
  % & $C_{5,2}^{+}$ & $v_{10} \rightarrow v_5 \rightarrow v_7 \rightarrow v_{10}$
  % \\ \hline
  % \multirow{1}{*}{$\mathcal{M}_6$} & $\gamma_6^{+}$
  % & $C_6^{+}$ & $v_2 \rightarrow v_2$
  \\ \hline
  \multirow{1}{*}{$\mathcal{M}_6$} & $\gamma_6^{1-}$
  & $e_1 \rightarrow e_{13} \rightarrow e_{14}$
  & no 
  & - & -
  \\ \hline
\end{tabular}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../MARS-n2D"
%%% End:


==> tab/table6.1.tex <==
\begin{tabular}{c|c|ccccc}
  % T = 4
  \hline \hline
  \multicolumn{2}{c|}{Results based on $\sum_{i = 1}^5 E_i$}
  & $h = \frac{1}{32}$
  & rate & $h = \frac{1}{64}$   & rate & $h = \frac{1}{128}$  \\
  \hline
  \multirow{3}{*}{\makecell{$T = 4$, \\ constant ARMS
  \\ with $r_{\Tiny}=0.05$}}
  &$h_L=0.2h$ & 2.53e-09 &  3.94 &  1.65e-10 &  3.98 &  1.05e-11 \\
  \cline{2-7}
  &$h_L=1.5h^{\frac{3}{2}}$ & 8.29e-09 &  6.03 &  1.27e-10 &  5.95 &  2.05e-12 \\
  \cline{2-7}
  &$h_L=10h^2$ & 1.67e-08 &  8.08 &  6.16e-11 &  7.75 &  2.87e-13 \\
  \hline
  % T = 8
  \multirow{3}{*}{\makecell{$T = 8$, \\ constant ARMS
  \\ with $r_{\Tiny}=0.01$}}
  &$h_L=0.2h$ & 8.70e-09 &  4.19 &  4.77e-10 &  3.97 &  3.05e-11 \\
  \cline{2-7}
  &$h_L=1.5h^{\frac{3}{2}}$ & 3.81e-08 &  6.68 &  3.71e-10 &  5.97 &  5.92e-12 \\
  \cline{2-7}
  &$h_L=10h^2$ & 7.56e-08 &  8.74 &  1.77e-10 &  7.93 &  7.24e-13 \\
  \hline
  % T = 12
  \multirow{3}{*}{\makecell{$T = 12$, \\ curvature-based ARMS  \\
  {\small with (\ref{eq:vortex-test-parametersCB}) \& $r_{\min}^c=0.01$}}}
  &$h_L^c=0.2h$ & 1.77e-09 &  3.88 &  1.20e-10 &  3.99 &  7.59e-12  \\
  \cline{2-7}
  &$h_L^c=1.5h^{\frac{3}{2}}$ & 4.75e-09 &  5.83 &  8.32e-11 &  6.15 &  1.17e-12 \\
  \cline{2-7}
  &$h_L^c=10h^2$ & 9.81e-09 &  7.93 &  4.03e-11 &  7.54 &  2.17e-13 \\
  \hline
  % T = 16
  \multirow{3}{*}{\makecell{$T = 16$, \\ curvature-based ARMS  \\
  {\small with (\ref{eq:vortex-test-parametersCB})
  \& $r_{\min}^c=0.005$}}}
  &$h_L^c=0.2h$ & 2.19e-09 &  3.82 &  1.56e-10 &  4.16 &  8.74e-12 \\
  \cline{2-7}
  &$h_L^c=1.5h^{\frac{3}{2}}$ & 7.39e-09 &  5.98 &  1.17e-10 &  6.21 &  1.59e-12 \\
  \cline{2-7}
  &$h_L^c=10h^2$ & 1.27e-08 &  8.08 &  4.69e-11 &  7.57 &  2.47e-13 \\
  % Each phase
  \hline \hline
  Results based on $E_i$ & phase & $h = \frac{1}{32}$
  & rate & $h = \frac{1}{64}$   & rate & $h = \frac{1}{128}$  \\
  \hline
  \multirow{5}{*}{\makecell{$T = 16$, \\ curvature-based ARMS \\
  with $h_L^c=0.2h$, \\
  (\ref{eq:vortex-test-parametersCB}), and $r_{\min}^c=0.005$}}
  &blue  & 5.23e-10 &  3.74 &  3.91e-11 &  4.18 &  2.16e-12 \\
  \cline{2-7}
  &cyan  & 4.70e-10 &  3.90 &  3.15e-11 &  4.11 &  1.83e-12 \\
  \cline{2-7}
  &red   & 3.08e-10 &  4.03 &  1.88e-11 &  4.18 &  1.04e-12 \\
  \cline{2-7}
  &green & 3.17e-10 &  3.53 &  2.75e-11 &  4.24 &  1.45e-12 \\
  \cline{2-7}
  &white & 5.78e-10 &  3.90 &  3.88e-11 &  4.10 &  2.26e-12 \\
  \hline \hline
\end{tabular}


==> tab/table6.2.tex <==
\begin{tabular}{c|ccccc}
  % Comparison T1
  \hline \hline
  \multicolumn{6}{l}{(a): the three-phase vortex-shear test
  in \cite[Sec. 3.5]{sijoy2010volume} with $T=8$}\\
  \hline
  method  & $h = \frac{1}{32}$ & rate
  & $h = \frac{1}{64}$ & rate & $h = \frac{1}{128}$
  \\ \hline
  constant ARMS & 3.44e-09 & 3.97 & 2.19e-10 & 3.96 & 1.41e-11
  \\ \hline
  LV + NI & 3.21e-02 & 1.16 & 1.44e-02 & 1.22 & 6.16e-03 \\ \hline
  LV + MC & 2.91e-02 & 1.17 & 1.29e-02 & 1.10 & 6.02e-03 \\ \hline
  LV + MB & 2.28e-02 & 1.05 & 1.11e-02 & 0.89 & 5.95e-03
  \\
  \hline \hline
  \multicolumn{6}{l}{(b): the two-phase vortex-shear test
  in \cite[Sec. 4.3]{hergibo2023moment} with $T=8$}\\ \hline
  method  & $h = \frac{1}{32}$ & rate
  & $h = \frac{1}{64}$ & rate & $h = \frac{1}{128}$
  \\ \hline
  constant ARMS
          & 4.58e-09 & 3.82 & 3.24e-10 & 3.92 & 2.13e-11
  \\ \hline
  Standard MOF
          & 1.42e-02 & 0.92 & 7.46e-03 & 2.53 & 1.29e-03 \\ \hline
  MOF by Jemison \cite{jemison2015:_filament}
          & 3.12e-03 & 2.17 & 6.91e-04 & 1.31 & 2.77e-04 \\
  % MOF by Hergibo et al. \cite{hergibo2023moment}
  %         & 2.80e-03 & 2.46 & 5.06e-04 & 1.71 & 1.54e-04 \\
  \hline \hline
  \multicolumn{6}{l}{(c): the two-phase vortex-shear test
  in \cite[Sec. 4.4]{hergibo2023moment} with $T=12$}
  % \\ \hline
  % method  & $h = \frac{1}{32}$ & rate
  % & $h = \frac{1}{64}$ & rate & $h = \frac{1}{128}$
  \\ \hline
  method  & $h = \frac{1}{32}$ & rate
  & $h = \frac{1}{64}$ & rate & $h = \frac{1}{128}$
  \\ \hline
  curvature-based ARMS & 1.07e-09 & 3.87 & 7.33e-11 & 3.96 & 4.72e-12\\ \hline
  standard MOF for two phases
          & 2.66e-02 & 0.55 & 1.81e-02 & 2.42 & 3.37e-03 \\ \hline
  MOF by Hergibo et al. \cite{hergibo2023moment}
          & 4.98e-03 & 2.32 & 9.91e-04 & 1.99 & 2.48e-04 \\
  \hline \hline
\end{tabular}

==> tab/table6.3.tex <==
\begin{tabular}{c|c|ccccc}
  % T = 2
  \hline \hline
  Results based on $\sum_{i = 1}^6 E_i$ & $h_L^c$  & $h = \frac{1}{32}$
                                  & rate              & $h = \frac{1}{64}$ & rate & $h = \frac{1}{128}$                   \\
  \hline
  \multirow{3}{*}{\makecell{$T = 2$,                                                                                      \\ curvature-based ARMS
  \\ with (\ref{eq:curvatureStrategyConstants}) and $r_{\min}^c = 0.1$}}
                                  & $0.2h$            & 4.45e-09 &  3.88 &  3.03e-10 &  4.07 &  1.81e-11 \\
  \cline{2-7}
                                  & $1.5h^{\frac{3}{2}}$ & 1.35e-08 &  5.91 &  2.25e-10 &  6.02 &  3.46e-12 \\
  \cline{2-7}
                                  & $10h^2$          & 2.68e-08 &  8.02 &  1.04e-10 &  7.93 &  4.25e-13 \\
  \hline
  % T = 4
  \multirow{3}{*}{\makecell{$T = 4$,                                                                                      \\ curvature-based ARMS
  \\ with (\ref{eq:curvatureStrategyConstants}) and $r_{\min}^c = 0.05$}}
                                  & $0.2h$            & 5.62e-09 &  3.99 &  3.54e-10 &  4.03 &  2.16e-11 \\
  \cline{2-7}
                                  & $1.5h^{\frac{3}{2}}$ & 1.45e-08 &  5.92 &  2.41e-10 &  6.03 &  3.68e-12 \\
  \cline{2-7}
                                  & $10h^2$          & 2.85e-08 &  8.03 &  1.09e-10 &  8.20 &  3.72e-13 \\
  \hline \hline
  Results based on $E_i$ & phase & $h = \frac{1}{32}$
  & rate & $h = \frac{1}{64}$   & rate & $h = \frac{1}{128}$  \\
  \hline
  \multirow{4}{*}{\makecell{$T = 4$, \\ curvature-based ARMS \\
  with $h_L^c=0.2h$, \\
  (\ref{eq:curvatureStrategyConstants}), and $r_{\min}^c=0.05$}}
  &blue  & 7.38e-10 & 4.01 & 4.58e-11 & 3.99 & 2.88e-12 \\
  \cline{2-7}
  % &cyan  & 7.38e-10 & 4.01 & 4.58e-11 & 3.99 & 2.88e-12 \\
  % \cline{2-7}
  &red  & 5.32e-10 & 4.08 & 3.14e-11 & 3.91 & 2.09e-12 \\
  \cline{2-7}
  &green & 1.05e-09 & 3.77 & 7.65e-11 & 3.99 & 4.80e-12 \\
  \cline{2-7}
  % &pink  & 5.32e-10 & 4.08 & 3.14e-11 & 3.91 & 2.09e-12 \\
  % \cline{2-7}
  &white & 2.04e-09 & 4.07 & 1.22e-10 & 4.14 & 6.89e-12 \\
  \hline \hline
\end{tabular}

==> tab/table6.4.tex <==
\begin{tabular}{c|c|ccccc}
  \hline \hline
  method             & phase & $h = \frac{1}{32}$            & rate & $h = \frac{1}{64}$            & rate & $h = \frac{1}{128}$            \\
  \hline
  %    \multirow{6}{*}{\makecell{constant ARMS
  \multirow{4}{*}{\makecell{constant ARMS
  \\ with $k = \frac{1}{8}h$ and \\
      $(r_{\mathrm{tiny}},h_L) = (0.005, 0.2h)$}}
                     & blue  & 5.70e-08 &  4.23 &  3.03e-09 &  5.31 &  7.66e-11                       \\
  \cline{2-7}
  % & cyan   & 5.70e-08 &  4.23 &  3.03e-09 &  5.31 &  7.66e-11 \\
                     & red   & 1.09e-08 &  4.03 &  6.64e-10 &  3.63 &  5.35e-11                       \\
  \cline{2-7}
                     & green & 1.88e-08 &  3.97 &  1.20e-09 &  3.98 &  7.55e-11                       \\
  \cline{2-7}
  %     & pink   & 1.05e-08 &  3.99 &  6.60e-10 &  3.64 &  5.29e-11 \\
                     & white & 1.21e-07 &  4.25 &  6.40e-09 &  5.19 &  1.75e-10                       \\
  \hline
  \multirow{4}{*}{\makecell{curvature-based ARMS
  \\ with $k = \frac{1}{8}h$, $h_L^c = 0.2 h$, \\
      (\ref{eq:curvatureStrategyConstants}), and $r_{\min}^c = 0.1$.}}
                     & blue  & 5.80e-10 &  3.81 &  4.12e-11 &  4.17 &  2.28e-12                       \\
  \cline{2-7}
  % & cyan   & 5.54e-10 &  3.93 &  3.63e-11 &  4.18 &  2.00e-12 \\
                     & red   & 4.55e-10 &  4.05 &  2.75e-11 &  4.08 &  1.62e-12                       \\
  \cline{2-7}
                     & green & 9.08e-10 &  3.69 &  7.03e-11 &  3.91 &  4.67e-12                       \\
  \cline{2-7}
  %     & pink   & 4.60e-10 &  4.06 &  2.75e-11 &  4.08 &  1.63e-12 \\
                     & white & 1.50e-09 &  3.91 &  9.97e-11 &  4.08 &  5.88e-12                       \\
  \hline
  \multirow{4}{*}{\makecell{curvature-based ARMS
  \\ with $k = h$, $h_L^c = 0.2 h$, \\
      (\ref{eq:curvatureStrategyConstants}), and $r_{\min}^c = 0.1$.}}
                     & blue  & 3.20e-06                      & 4.84 & 1.12e-07                      & 5.00 & 3.51e-09                       \\
  \cline{2-7}
  % & cyan  & 3.20e-06 &  4.84 &  1.12e-07 &  5.00 &  3.51e-09 \\
                     & red   & 4.23e-06                      & 4.98 & 1.34e-07                      & 4.99 & 4.24e-09                       \\
  \cline{2-7}
                     & green & 2.98e-06                      & 4.96 & 9.57e-08                      & 5.00 & 3.00e-09                       \\
  \cline{2-7}
  %     & pink  & 4.23e-06 &  4.98 &  1.34e-07 &  4.99 &  4.24e-09 \\
                     & white & 6.97e-06                      & 4.97 & 2.22e-07                      & 5.00 & 6.96e-09                       \\
  \hline \hline
  $t = \frac{1}{2}T$ & phase & $\frac{1}{16} - \frac{1}{32}$ & rate & $\frac{1}{32} - \frac{1}{64}$ & rate & $\frac{1}{64} - \frac{1}{128}$ \\
  \hline
  \multirow{4}{*}{\makecell{curvature-based ARMS
  \\ with $k = \frac{1}{8}h$, $h_L^c = 0.2 h$, \\
      (\ref{eq:curvatureStrategyConstants}), and $r_{\min}^c = 0.1$.}}
                     & blue  & 1.36e-08 &  3.57 &  1.15e-09 &  3.91 &  7.62e-11                      \\
  \cline{2-7}
  % & cyan  & 1.36e-08 &  3.57 &  1.15e-09 &  3.91 &  7.62e-11 \\
                     & red   & 1.38e-08 &  3.82 &  9.74e-10 &  3.75 &  7.26e-11                       \\
  \cline{2-7}
                     & green & 2.10e-08 &  3.93 &  1.37e-09 &  3.84 &  9.58e-11                       \\
  \cline{2-7}
  %     & pink  & 1.38e-08 &  3.82 &  9.74e-10 &  3.75 &  7.26e-11 \\
                     & white & 4.76e-08 &  3.89 &  3.21e-09 &  4.05 &  1.94e-10                       \\
  \hline \hline
\end{tabular}

==> tab/table6.5.tex <==
\begin{tabular}{c|ccccc}
  \hline \hline
  method  & $h = \frac{1}{32}$ & rate & $h = \frac{1}{64}$ & rate & $h = \frac{1}{128}$ \\
  \hline
  curvature-based
  ARMS    & 2.71e-09           & 3.91 & 1.80e-10           & 4.05 & 1.09e-11           \\
  \hline
  LV + NI & 3.05e-02           & 0.92 & 1.61e-02           & 1.39 & 6.13e-03            \\
  \hline
  LV + MC & 2.37e-02           & 0.80 & 1.37e-02           & 1.16 & 6.10e-03            \\
  \hline
  LV + MB & 2.10e-02           & 0.76 & 1.25e-02           & 1.05 & 6.00e-03            \\
  \hline \hline
\end{tabular}

==> tab/table6.6.tex <==
\begin{tabular}{c|c|ccccc}
  % T = 2
  \hline \hline
  Results based on $\sum_{i = 1}^6 E_i$ & $h_L^c$  & $h = \frac{1}{32}$
                                  & rate              & $h = \frac{1}{64}$ & rate & $h = \frac{1}{128}$                   \\
  \hline
  \hline
  \multirow{3}{*}{\makecell{Vortex, $T_v = 4$, \\ curvature-based ARMS  \\
  {\small with (\ref{eq:curvatureStrategyGraphVortex}) \& $r_{\min}^c=0.02$}}}
  &$0.2h$ & 3.48e-10 &  3.95 &  2.25e-11 &  3.84 &  1.58e-12 \\
  \cline{2-7}
  &$1.5h^{\frac{3}{2}}$ & 1.20e-09 &  6.25 &  1.57e-11 &  5.88 &  2.68e-13 \\
  \cline{2-7}
  &$10h^2$ & 2.18e-09 &  7.86 &  9.40e-12 &  6.99 &  7.40e-14  \\
  \hline
  % T = 8
  \multirow{3}{*}{\makecell{Vortex, $T_v = 8$, \\ curvature-based ARMS  \\
  {\small with (\ref{eq:curvatureStrategyGraphVortex}) \& $r_{\min}^c=0.02$}}}
  &$0.2h$ & 1.70e-09 &  3.86 &  1.17e-10 &  3.92 &  7.73e-12 \\
  \cline{2-7}
  &$1.5h^{\frac{3}{2}}$ & 5.70e-09 &  6.04 &  8.69e-11 &  5.93 &  1.43e-12 \\
  \cline{2-7}
  &$10h^2$ &  9.65e-09 &  7.82 &  4.27e-11 &  7.61 &  2.19e-13 \\
  \hline
  % T = 12
  \multirow{3}{*}{\makecell{Vortex, $T_v = 12$, \\ curvature-based ARMS  \\
  {\small with (\ref{eq:curvatureStrategyGraphVortex}) \& $r_{\min}^c=0.01$}}}
  &$0.2h$ & 4.38e-09 &  4.23 &  2.34e-10 &  4.03 &  1.43e-11 \\
  \cline{2-7}
  &$1.5h^{\frac{3}{2}}$ & 1.07e-08 &  5.88 &  1.82e-10 &  6.06 &  2.73e-12 \\
  \cline{2-7}
  &$10h^2$ &2.04e-08 &  8.00 &  7.97e-11 &  7.60 &  4.11e-13 \\
  \hline
  % T = 16
  \multirow{3}{*}{\makecell{Vortex, $T_v = 16$, \\ curvature-based ARMS  \\
  {\small with (\ref{eq:curvatureStrategyGraphVortex})
  \& $r_{\min}^c=0.005$}}}
  &$0.2h$ & 6.08e-09 &  4.28 &  3.14e-10 &  4.15 &  1.76e-11 \\
  \cline{2-7}
  &$1.5h^{\frac{3}{2}}$ & 1.42e-08 &  6.13 &  2.01e-10 &  5.73 &  3.80e-12 \\
  \cline{2-7}
  &$10h^2$ & 2.57e-08 &  8.07 &  9.53e-11 &  7.54 &  5.11e-13 \\
  \hline
  % Deformation, T = 2
  \multirow{3}{*}{\makecell{Deformation, $T_d = 2$,                                                                                      \\ curvature-based ARMS
  \\ with (\ref{eq:curvatureStrategyGraphDeformation}) \&  $r_{\min}^c = 0.1$}}
                                  & $0.2h$            & 1.32e-08 &  3.91 &  8.79e-10 &  3.94 &  5.73e-11 \\
  \cline{2-7}
                                  & $1.5h^{\frac{3}{2}}$ & 4.05e-08 &  5.91 &  6.75e-10 &  5.98 &  1.07e-11 \\
  \cline{2-7}
                                  & $10h^2$          & 8.18e-08 &  7.93 &  3.35e-10 &  8.03 &  1.28e-12 \\
  \hline
  % T = 4
  \multirow{3}{*}{\makecell{Deformation, $T_d = 4$,                                                                                      \\ curvature-based ARMS
  \\ with (\ref{eq:curvatureStrategyGraphDeformation}) \&  $r_{\min}^c = 0.01$}}
                                  & $0.2h$            & 1.45e-08 &  3.99 &  9.10e-10 &  4.11 &  5.25e-11 \\
  \cline{2-7}
                                  & $1.5h^{\frac{3}{2}}$ & 3.98e-08 &  6.01 &  6.15e-10 &  5.94 &  1.00e-11 \\
  \cline{2-7}
                                  & $10h^2$          & 8.06e-08 &  7.99 &  3.18e-10 &  7.86 &  1.37e-12 \\
  \hline \hline
  Results based on $E_i$ & phase & $h = \frac{1}{32}$
  & rate & $h = \frac{1}{64}$   & rate & $h = \frac{1}{128}$  \\
  \hline
  \multirow{6}{*}{\makecell{Vortex, $T_v = 16$, \\ curvature-based ARMS \\
  with $h_L^c=0.2h$, \\
  (\ref{eq:curvatureStrategyGraphVortex}), and $r_{\min}^c=0.005$}}
  &blue  & 3.62e-10 &  4.14 &  2.06e-11 &  4.46 &  9.34e-13 \\
  \cline{2-7}
  &cyan  & 2.38e-10 &  4.30 &  1.20e-11 &  4.41 &  5.64e-13 \\
  \cline{2-7}
  &red  & 2.95e-10 &  4.80 &  1.06e-11 &  4.26 &  5.52e-13 \\
  \cline{2-7}
  &green & 2.80e-09 &  4.31 &  1.41e-10 &  4.12 &  8.10e-12 \\
  \cline{2-7}
  &pink  & 1.17e-09 &  4.88 &  3.97e-11 &  3.98 &  2.51e-12 \\
  \cline{2-7}
  &white & 1.22e-09 &  3.76 &  8.97e-11 &  4.17 &  4.98e-12 \\
  \hline
  \multirow{6}{*}{\makecell{Deformation, $T_d = 4$, \\ curvature-based ARMS \\
  with $h_L^c=0.2h$, \\
  (\ref{eq:curvatureStrategyGraphDeformation}), and $r_{\min}^c=0.01$}}
  &blue  & 7.43e-10 &  4.07 &  4.43e-11 &  4.21 &  2.40e-12 \\
  \cline{2-7}
  &cyan  & 8.63e-10 &  3.97 &  5.50e-11 &  4.19 &  3.01e-12 \\
  \cline{2-7}
  &red  & 8.42e-10 &  4.01 &  5.24e-11 &  4.23 &  2.79e-12 \\
  \cline{2-7}
  &green & 6.45e-09 &  4.02 &  3.97e-10 &  4.09 &  2.32e-11 \\
  \cline{2-7}
  &pink  & 2.25e-09 &  3.84 &  1.57e-10 &  4.14 &  8.88e-12 \\
  \cline{2-7}
  &white & 3.35e-09 &  4.03 &  2.05e-10 &  4.07 &  1.22e-11 \\
  \hline \hline
\end{tabular}



==> tab/table6.7.tex <==
\begin{tabular}{c|c|ccccc}
  % T = 12
  \hline \hline
  Results based on $\sum_{i = 1}^{22} E_i$ & $h_L^c$  & $h = \frac{1}{32}$
                                  & rate              & $h = \frac{1}{64}$ & rate & $h = \frac{1}{128}$                   \\
  \hline
  \multirow{3}{*}{\makecell{Vortex, $T_v = 12$, \\ curvature-based ARMS  \\
  {\small with (\ref{eq:curvatureStrategyGraphVortex})
  \& $r_{\min}^c=0.01$}}}
                                  & $0.2h$            & 6.84e-08 &  3.62 &  5.58e-09 &  3.94 &  3.64e-10 \\
  \cline{2-7}
                                  & $1.5h^{\frac{3}{2}}$ & 1.77e-07 &  5.43 &  4.11e-09 &  5.94 &  6.70e-11 \\
  \cline{2-7}
                                  & $10h^2$          & 3.29e-07 &  7.35 &  2.01e-09 &  7.72 &  9.54e-12 \\
  \hline
  % T = 16
  \multirow{3}{*}{\makecell{Vortex, $T_v = 16$, \\ curvature-based ARMS  \\
  {\small with (\ref{eq:curvatureStrategyGraphVortex})
  \& $r_{\min}^c=0.005$}}}
                                  & $0.2h$            & 8.18e-08 &  3.82 &  5.78e-09 &  3.83 &  4.05e-10 \\
  \cline{2-7}
                                  & $1.5h^{\frac{3}{2}}$ & 2.01e-07 &  5.43 &  4.66e-09 &  5.89 &  7.84e-11 \\
  \cline{2-7}
                                  & $10h^2$          & 3.94e-07 &  7.54 &  2.11e-09 &  7.56 &  1.12e-11 \\
  \hline
  % T = 2
  \multirow{3}{*}{\makecell{Deformation, $T_d = 2$,                                                                                      \\ curvature-based ARMS
  \\ with (\ref{eq:curvatureStrategyGraphDeformation}) \&  $r_{\min}^c = 0.05$}}
                                  & $0.2h$            & 1.65e-08 &  3.74 &  1.23e-09 &  3.71 &  9.38e-11 \\
  \cline{2-7}
                                  & $1.5h^{\frac{3}{2}}$ & 5.88e-08 &  5.98 &  9.28e-10 &  5.79 &  1.68e-11 \\
  \cline{2-7}
                                  & $10h^2$          & 8.52e-08 &  7.54 &  4.57e-10 &  7.57 &  2.40e-12 \\
  \hline \hline
\end{tabular}


==> tab/tableCpu1.tex <==
\begin{tabular}{c|c|ccccc}
  % T = 2
  \hline \hline
  CPU time (s) & $h_L^c$  & $h = \frac{1}{32}$
                                  & rate              & $h = \frac{1}{64}$ & rate & $h = \frac{1}{128}$                   \\
  \hline
  \multirow{3}{*}{\makecell{$T = 2$,                                                                                      \\ curvature-based ARMS
  \\ with (\ref{eq:curvatureStrategyConstants}) and $r_{\min}^c = 0.1$}}
                                  & $0.2h$            & 4.27e+00 &  1.95 &  1.65e+01 &  1.98 &  6.49e+01 \\
  \cline{2-7}
                                  & $1.5h^{\frac{3}{2}}$ & 3.65e+00 &  2.47 &  2.01e+01 &  2.76 &  1.37e+02 \\
  \cline{2-7}
                                  & $10h^2$          & 3.87e+00 &  2.97 &  3.03e+01 &  3.12 &  2.63e+02 \\
  \hline
  % T = 4
  \multirow{3}{*}{\makecell{$T = 4$,                                                                                      \\ curvature-based ARMS
  \\ with (\ref{eq:curvatureStrategyConstants}) and $r_{\min}^c = 0.05$}}
                                  & $0.2h$            & 2.13e+01 &  2.03 &  8.69e+01 &  2.14 &  3.82e+02 \\
  \cline{2-7}
                                  & $1.5h^{\frac{3}{2}}$ & 1.85e+01 &  2.59 &  1.11e+02 &  2.72 &  7.30e+02\\
  \cline{2-7}
                                  & $10h^2$          & 1.85e+01 &  3.14 &  1.63e+02 &  3.37 &  1.68e+03 \\
  \hline \hline
\end{tabular}

==> tab/tableCpu2.tex <==
\begin{tabular}{c|c|ccccc}
  % T = 12
  \hline \hline
  CPU time (s)  & $h_L^c$ & $h = \frac{1}{32}$
                                  & rate              & $h = \frac{1}{64}$ & rate & $h = \frac{1}{128}$                   \\
  \hline
  \multirow{3}{*}{\makecell{Vortex, $T_v = 12$, \\ curvature-based ARMS  \\
  {\small with (\ref{eq:curvatureStrategyGraphVortex})
  \& $r_{\min}^c=0.01$}}}
                                  & $0.2h$            & 7.95e+01 &  1.74 &  2.65e+02 &  1.92 &  1.00e+03 \\
  \cline{2-7}
                                  & $1.5h^{\frac{3}{2}}$ & 6.61e+01 &  2.22 &  3.09e+02 &  2.55 &  1.80e+03 \\
  \cline{2-7}
                                  & $10h^2$          & 6.89e+01 &  2.75 &  4.64e+02 &  3.04 &  3.82e+03 \\
  \hline
  % T = 16
  \multirow{3}{*}{\makecell{Vortex, $T_v = 16$, \\ curvature-based ARMS  \\
  {\small with (\ref{eq:curvatureStrategyGraphVortex})
  \& $r_{\min}^c=0.005$}}}
                                  & $0.2h$            & 1.15e+02 &  1.85 &  4.16e+02 &  1.99 &  1.65e+03 \\
  \cline{2-7}
                                  & $1.5h^{\frac{3}{2}}$ & 1.04e+02 &  2.24 &  4.91e+02 &  2.55 &  2.87e+03 \\
  \cline{2-7}
                                  & $10h^2$          & 1.03e+02 &  2.70 &  6.71e+02 &  3.17 &  6.04e+03 \\
  \hline
  % T = 2
  \multirow{3}{*}{\makecell{Deformation, $T_d = 2$,                                                                                      \\ curvature-based ARMS
  \\ with (\ref{eq:curvatureStrategyGraphDeformation}) \&  $r_{\min}^c = 0.05$}}
                                  & $0.2h$            & 3.72e+01 &  1.98 &  1.47e+02 &  2.07 &  6.18e+02 \\
  \cline{2-7}
                                  & $1.5h^{\frac{3}{2}}$ &3.15e+01 &  2.46 &  1.73e+02 &  2.72 &  1.14e+03 \\
  \cline{2-7}
                                  & $10h^2$          & 3.20e+01 &  3.00 &  2.57e+02 &  3.30 &  2.53e+03 \\
  \hline \hline
\end{tabular}



==> tab/tablePig.tex <==
\begin{tabular}{c|c|ccccc}
  % T = 12
  \hline \hline
  Results based on $\sum_{i = 1}^{15} E_i$ & $h_L^c$  & $h = \frac{1}{32}$
                                  & rate              & $h = \frac{1}{64}$ & rate & $h = \frac{1}{128}$                   \\
  \hline
  
  \multirow{3}{*}{\makecell{Vortex, $T = 4$, \\ curvature-based ARMS  \\
  {\small with (\ref{eq:curvatureStrategyGraphVortex}) \& $r_{\min}^c=0.02$}}}
                                  & $0.1h$            & 1.95e-08 &  4.05 &  1.17e-09 &  3.71 &  8.99e-11 \\
  \cline{2-7}
                                  & $0.75h^{\frac{3}{2}}$ & 3.36e-08 &  5.36 &  8.20e-10 &  5.30 &  2.09e-11  \\
  \cline{2-7}
                                  & $5h^2$          & 9.05e-08 &  7.82 &  4.01e-10 &  7.60 &  2.07e-12 \\
  \hline
  % T = 16
  \multirow{3}{*}{\makecell{Vortex, $T = 8$, \\ curvature-based ARMS  \\
  {\small with (\ref{eq:curvatureStrategyGraphVortex}) \& $r_{\min}^c=0.02$}}}
                                  & $0.1h$            & 8.03e-08 &  5.16 &  2.25e-09 &  3.62 &  1.83e-10 \\
  \cline{2-7}
                                  & $0.75h^{\frac{3}{2}}$ &  1.24e-07 &  6.38 &  1.49e-09 &  5.21 &  4.02e-11 \\
  \cline{2-7}
                                  & $5h^2$          & 2.53e-07 &  7.47 &  1.43e-09 &  7.08 &  1.06e-11 \\
  \hline \hline
\end{tabular}

